Learning at the Speed of Wireless: Online Real-Time Learning for AI-Enabled MIMO in NextG

Integration of artificial intelligence (AI) and machine learning (ML) into the air interface has been envisioned as a key technology for next-generation (NextG) cellular networks. At the air interface, multiple-input multiple-output (MIMO) and its variants such as multi-user MIMO (MU-MIMO) and massive/full-dimension MIMO have been key enablers across successive generations of cellular networks with evolving complexity and design challenges. Initiating active investigation into leveraging AI/ML tools to address these challenges for MIMO becomes a critical step towards an AI-enabled NextG air interface. At the NextG air interface, the underlying wireless environment will be extremely dynamic with operation adaptations performed on a sub-millisecond basis by MIMO operations such as MU-MIMO scheduling and rank/link adaptation. Given the enormously large number of operation adaptation possibilities, we contend that online real-time AI/ML-based approaches constitute a promising paradigm. To this end, we outline the inherent challenges and offer insights into the design of such online real-time AI/ML-based solutions for MIMO operations. An online real-time AI/ML-based method for MIMO-OFDM channel estimation is then presented, serving as a potential roadmap for developing similar techniques across various MIMO operations in NextG.

==> figures/mse_var_channel_estimation.tex <==
\begin{figure}[t] 
    \centering
    \includegraphics[width=1\linewidth] {Figure/NMSE2x2_var.pdf}
    \caption{Variance of Normalized mean square error (NMSE) of channel estimation methods. 
    % The ``em-LMMSE" denotes empirical LMMSE. 
    % The ``ReEsNet (mismatch)" represents ReEsNet with offline and online data distribution mismatch.
    % ReEsNet with offline and online data distribution mismatch is shown as ``ReEsNet (mismatch)". 
    }
    \label{fig:MSE_var}
\end{figure}

==> figures/pilot_pattern.tex <==
\begin{figure}[t] 
    \centering
    \includegraphics[width=1\linewidth] {Figure/pilot_pattern.pdf}
    \caption{Pilot patterns for conventional and learning-based methods. 
    }
    \label{fig:pilot_pattern}
\end{figure}

==> tables/existing_work.tex <==
\begin{table}[]
\centering
\caption{Overview of AI/ML-enabled approaches from offline learning to online learning}
\label{tab:applications comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c l l l l }
\toprule
   &     Applications              & Offline              & Hybrid      & Online              \\
 \midrule
Transmitter & Precoding \& Beam Management          & DNN~\cite{Hojatian2021} &     DNN~\cite{Yuan2021_BM_Transfer_Learning}        &    DRL~\cite{9804217}   \\
 & Scheduling \& Multiple Access        &   DNN~\cite{Cerna2023}                   &           & DRL~\cite{Mauricio2022}\\
 % & mmWave Beam Management & RNN \cite{Ma2021_BeamMgmt}  &   & DRL~\cite{Zhang2021_BeamMgmt} \\
\midrule
% Receiver & Channel Estimation & CNN~\cite{CLiu2022}, DNN~\cite{LLi2020}       &         DNN~\cite{RoemNet}    & DNN~\cite{XZheng2021}, DRL~\cite{MOh2021} \\
Receiver & Channel Estimation & DNN~\cite{LLi2020}       &          & DNN~\cite{XZheng2021, li2023learning}, DRL~\cite{MOh2021} \\
 % & Symbol Detection   &   DNN~\cite{samuel2019detnet}      & DNN~\cite{Shlezinger2020ViterbiNet}          & RNN~\cite{JXu2023}                             \\
  & Symbol Detection   &        &           & RNN~\cite{JXu2023}                             \\
 & Channel Prediction     &                      &    DNN~\cite{Yang2020DeepTransfer}        & RNN~\cite{8801923}, DRL~\cite{9804217}              \\
\midrule
CSI Feedback & CSI Compression    & DNN~\cite{wen2018csinet}        & DNN~\cite{9803260}  & -  \\
\bottomrule
\end{tabular}%
}
\end{table}

